Encoding Schemes for Parallel In-Place Algorithms

Many parallel algorithms which solve basic problems in computer science use auxiliary space linear in the input to facilitate conflict-free computation. There has been significant work on improving these parallel algorithms to be in-place, that is to use as little auxiliary memory as possible. In this paper, we provide novel in-place algorithms to solve the fundamental problems of merging two sorted sequences, and randomly shuffling a sequence. Both algorithms are work-efficient and have polylogarithmic span. Our algorithms employ encoding techniques which exploit the underlying structure of the input to gain access to more bits, which enables the use of auxiliary data as well as non-in-place methods. The encoding techniques we develop are general. We expect them to be useful in developing in-place algorithms for other problems beyond those already mentioned. To demonstrate this, we outline an additional application to integer sorting. In addition to our theoretical contributions, we implement our merging algorithm, and measure its memory usage and runtime.

==> Sections/morecomplicatedenc.tex <==
\section{More complicated encodings}\label{morecompencode}

\subsection{Units and encodings}

As is standard, let $I$ be an array of $n$ unique elements from a totally ordered universe.

\begin{defn}
    A \emph{$k$-unit} of $I$ is a contiguous subsequence of length $k$.
\end{defn}

There is a natural way to decompose $I$ into units. We simply split $I$ into successive subsequences of length $k$. We think of this decomposition as defining an array $U$ of $n/k$ units where $U[p] = I[pk..p(k+1)-1]$. We refer to $U$ as the \emph{unit decomposition} for $I$. Because $I$ is totally ordered and unique, each $k$-unit can be permuted from its initial order to one of $k!$ possible ordering. We represent a permutation $\pi \colon [k] \rightarrow [k]$ by listing its values as follows:
\[[\pi(1),\pi(2),\dots,\pi(k)].\]
Denote the set of permutations of $k$ objects as $S_k$ and let $r \colon S_k \rightarrow \{0,1,\dots,k! - 1\}$ be given by
\[r(\pi,k) = (\pi(1) - 1)(k-1)! + r(\pi',k-1). \tag{1}\]
where
\[\pi'(i) = \begin{cases}
    \pi(i+1) - 1 & \text{ if } \pi(i+1) > \pi(1) \\
    \pi(i+1) & \text{ if } \pi(i+1) < \pi(1)
\end{cases}\]
Then the initial condition of the recurrence is $r([1],1) = 0$. $r(\pi,k)$ is said to be the rank of $\pi$. Note that $r$ is a bijection and $(1)$ is computable in $O(k^2)$ time using $O(k)$ space to store a factorial lookup table. Additionally, the inverse $r^{-1}(m)$ is similarly computable in $O(k^2)$ and $O(k)$ space to store a modulo lookup table (see section 2.4 of \cite{kreher_stinson_combinatorial_algorithms} for details).

Within each unit for $I$ we can encode values between $0$ and $k! - 1$ in the following manner. To \emph{write} a value $i$ to a unit $u$, we first compute $r^{-1}(i)$, then rearrange $u$ according to this permutation. This can be done by first sorting $u$ then applying the computed permutation to $u$. To \emph{read} a unit $u$, we first compute a list representation of its permutation through simulating a sort of $u$ and keeping track of the indices of its elements. We then use $r$ to compute its value. Both of these operations take $O(k^2)$ time and $k$ stack-allocated space.

\subsubsection{Typical encoding} \textcolor{blue}{In Progress...}

\subsection{Random Permutation}

In this section, we consider the random permutation problem; given an array $A$, randomly permute the elements of $A$. This problem has been studied extensively in the sequential setting, the out-of-place parallel setting \cite{10.5555/2722129.2722159}, and even the in-place parallel setting \cite{2021pip}. Our contribution is a substantial improvement of the main result of \cite{penschuck2023engineeringsharedmemoryparallelshuffling}, under the assumption that the elements of $A$ are taken from a totally ordered universe.

\begin{thm}
    Randomly permuting an array of size $n$ can be done using $O(n\log n)$ work and $O(\log^2 n \cdot \log \log n)$ depth whp using $O(\log n)$ sequential stack memory.
\end{thm}

Fix an an array $A$ of $n$ elements from a totally ordered universe. The following sequential algorithm produces a random permutation of $A$.

{%\footnotesize
\setlength{\interspacetitleruled}{0pt}%
\setlength{\algotitleheightrule}{0pt}%
\begin{algorithm2e}[ht]
\DontPrintSemicolon
\Fn {\mf{Knuth-Shuffle}(A)} {
\For {$i \leftarrow n$ to $1$} {
    $h \gets $ integer drawn uniformly random from $\{1,\dots, i\}$.\\
    swap($A[i]$, $A[h]$)
}
}
\end{algorithm2e}
}

This is an in-place version of the classical Knuth-shuffle algorithm; it will serve as the base case for our parallel algorithm. The following lemma provides a first step towards developing our algorithm.

\begin{lem}{\label{rperm-lemma}}
    Let $A$ be an array of $n$ elements and $(X_1,X_2,\dots,X_n)$ be a sequence of $n$ i.i.d. Bernoulli random variables with $p = 1/2$. Let $A_0 := \{ i \in A : X_i = 0\}$ and $A_1 := \{ i \in A : X_i = 1\}$, Also let $f$ be a permutation of $A$ that sends $A_0$ to $(1:|A_0|)$ and $A_1$ to $(|A_0|+1 : n)$. Further let $\bar \pi$ be the concatenation of two random permutations $\pi_0$ and $\pi_1$, where $\pi_0$ is a random permutation of $(1 : |A_0|)$ and $\pi_1$ is a random permutation of $(|A_0|+1 : n)$. Then $\pi := \bar \pi \circ f$ is a random permutation of $A$.
\end{lem}

We leave the proof of Lemma \ref{rperm-lemma} to the appendix. Guided by this fact, we can reduce the problem of generating a random permutation in-place to randomly partitioning an input array in-place, using the following algorithm.

\begin{algorithm2e}[H] 
\caption{PRp($A$,$i$,$j$) \Comment{Parallel in-place Random Permutation}}
\SetKwFor{ParFor}{parallel for}{do}{endfch}
\SetKwBlock{DoParallel}{do in parallel}{end}
\DontPrintSemicolon

\lIf{$|i-j| \leq N_0$}{Knuth-Shuffle($A[i:j]$) and return}
% \ParFor{$k \leftarrow i$ to $j$} {
%     $R[k] \gets$ uniform random integer from $\{0,1\}$ 
% }
% RandomPartition($A[i:j],R[i:j],P[\lceil i/b \rceil:\lfloor j/b \rfloor],i,j$) \\
$w \gets $ RandomPartition($A[i:j],n$) \Comment{$w$ is the splitting index of the partition} \\
\DoParallel  {
    PRp$(A,i,w)$  \\
    PRp$(A,w+1,j)$
}
\end{algorithm2e}
% \newpage

Executing $\text{PRp}(A,1,n)$ will randomly permute $A$. Lemma \ref{rperm-lemma} establishes the correctness of the algorithm. Also, PRp is in-place assuming that RandomPartition is in-place.

To obtain the in-place random partition algorithm, we modify the in-place partition algorithm given in \cite{kuszmaul2020inplaceparallelpartitionalgorithmsusing}. To facilitate the randomness, we require a more sophisticated encoding scheme. The encoding techniques we utilize are described at the beginning of this section.

We fix an array $X = (x_1,x_2,\dots,x_n)$ of length $n$. We will be using units of size $5$.
% Our encoding will require that the initial state of each unit be sorted. To ensure this we first sort the contiguous $5$ element subsequences of $X$, i.e. $X[1:5],X[6:10],\dots,X[k-4:k]$.
Next, we outline what data we need to encode implicitly. This consists of a random bit $r_i$ for each element $x_i$, and a prefix sum array $P$ which will assist in the partitioning step. To encode this information, we decompose $X$ into blocks $X_i$ of size $b = 5 \log n$, each split into a sequence of $\log n$ units of size $5$. Each unit can encode $6$ bits of information. Let $u_i = (x_{5i+1},x_{5i+2},\dots,x_{5i+5})$ be the $i$th unit of the decomposition and $(b_{i,1},\dots,b_{i,6})$ its associated bits. We use the first $5$ bits to encode the random bits for the elements of $u_i$. That is, $b_{i,j}$ encodes the random bit $r_{5i + j}$. For each block $B_i$, we are able to store another number $P[i]$ by encoding the $k$th bit of $P[i]$ using the last bit of the $k$th unit in $B_i$. Using the encode and decode operations described at the beginning of the section, the algorithm is as follows.

 \begin{algorithm2e}[H] 
\caption{RandomPartition($B$) \Comment{assuming $B$ is divisible by $b$}}\label{randompartition}
\SetKwFor{ParFor}{parallel for}{do}{endfch}
\SetKwFor{ParForEach}{parallel for each}{do}{endfch}
\SetKwBlock{DoParallel}{do in parallel}{end}
\DontPrintSemicolon

\ParForEach{unit $u_i$}{
    sort($u_i$) \\ 
    \For{$j = 1$ to $5$} {
        $r_{5i + j} \gets $ uniformly random element from $\{0,1\}$
    }
}

preprocess $B$ to make it successor heavy \Comment{described later}

\ParForEach{block $B_i$}{
    $P[k] \gets $ number of random bits which are 1 in block $B_i$ \Comment{number of successors in $B_i$}
}
compute implicit in-place parallel prefix sum on $P$ \Comment{as in [?]} \\
perform in-place reordering step \Comment{described later} \\
\textbf{return} splitting index $w$
\end{algorithm2e}

We describe how to do each step of Algorithm \ref{randompartition} in detail. \textcolor{blue}{In progress...}


We make $B$ successor heavy (line $4$) using a modified version of the recursive procedure given in [?]. Let $k = n/5$ and $U =(u_1,u_2,\dots,u_k)$ be the unit decomposition of $B$. We start with a parallel for loop: for each from $i = 1$ to $k/2$, we process the unit pair $u_i$ and $u_{k/2 + i}$ sequentially in the following manner: we first read the random bits $r_{i,0},\dots,r_{i,4}$ from $u_i$ and the random bits $r_{k/2 + i,0},\dots,r_{k/2 + i,4}$ from $u_{k/2+i}$ into the stack.

We elaborate more on line $8$. We follow the same procedure as in $[?]$ wherein we recurse on a prefix of $t$ blocks where $t$ is the smallest integer such that $t b > 4/5n$. Now in parallel for each block $B_j$ with $t < j \leq n/b$, we read the value of $P[j]$ and the random bits for each element in $B_j$ into the stack. We perform a parallel prefix sum in the stack on these bits to get values $s_a$ for each $a \in B_j$. Now using the random bits of each element in $B_j$ as the predicate function, we proceed as detailed in [?].

We outline how to modify the algorithm to accommodate arrays $B$ not divisible by $b$: We block $B$ as much as possible; on that sequence of blocks, we perform the algorithm above, so that part of $B$ is partitioned randomly. Thus, we only need to place the remaining elements into the partition. We do this sequentially: for each element in the remainder, we compute a random bit; if it is $0$, we swap with the element at the splitting index (the first element with random bit $1$) and update the splitting index.

Observe that the algorithm outlined above has essentially the same logical structure as that in [?], except with different read and write operations on units; these take $O(\log n)$ work and $O(\log \log n)$ depth by Lemma ?, which is the same as in [?], so the analysis there shows that RandomPartition takes $O(|B|)$ work and $O(\log |B| \log \log n)$ depth (the additional fixing step does not change this since there are $O(b)$ additional elements to process).
 
 % Run standard strong PIP partition algorithm, prepossessing is done unit by unit with the stack to handle corruption. Compute prefix sum using Strong PIP prefix sum. Other than that the algorithm follows the same structure of Strong pip partition modulo a few small changes.

% Let $b = 5\lceil \log n \rceil$ and block $A$ into $k = \lfloor n/b \rfloor$ blocks each of size $b$ expect possibly the last, which will be size $b + c$ where $c < b$. Denote these block as $B^1, B^2, \dots, B^k$. Further, for each $j < k$, we divide $B^j$ into $b / 5$ smaller blocks which we refer to as the units of $B^j$. Formally, each $B^j$ has $k_j = n/5$ units denoted $U^1,\dots,U^{k_j}$ each of size $5$. We divide block $B^k$ into $\lfloor (b+c)/5 \rfloor$ units each of size $5$ expect the last which has size at most $9$. We denote this special unit (in the sense that it is the only one whose size may be greater than $5$) as $U^s$. 

% Within each block, we can implicitly encode values through the relative ordering of its contents. Particularly, 

% \begin{lem}
%     Given a decomposition of $A$ into $k$ blocks of size at least $b$, there exists an encoding scheme to store at least $\frac{6}{5} \cdot n$ additional bits within $A$. Further, under this scheme $\log n$ bits can be encoded and decoded using $O(\log n)$ work, where encoding requires constant depth and decoding requires $O(\log\log n)$ depth.
% \end{lem}

% \begin{proof}
    
% \end{proof}


% There are two ways to achieve this. One is to use a PNRG (Pseudo Random Number Generator) to generate $R$ on the fly in $O(1)$ expected time. In order to guarantee repeatable results, we can store the generator's internal state either on the heap or in a threads local stack. The Mersenne Twister as an example, uses 32 bit seeds and requires $19968$ bits to store its internal state. Denote this version of Algorithm 1 as $\textit{PRpRg}$. Then we have the following:

\begin{thm}
    PRp is a strong PIP algorithm for Random Permutation using $O(n\log n)$ work and $O(\log^2 n \cdot \log \log n)$ depth whp.
\end{thm}
\begin{proof}
RandomPartition($B$) requires $O(|B|)$ work and $O(\log |B|  \log\log n) = O(\log n  \log\log n)$ depth. Thus at each level of the recursion, $O(n)$ work is done across all sub problems and each sub problem requires $O(\log n \cdot \log\log n)$ depth. Then it suffices to bound the recursive depth. In particular, we show that the recursive depth of PRp is $O(\log n)$ whp.

Let $a \in A$ and define $X_i$ to be the size of the sub problem that contains $a$ at the $i$th level of the recursion. Note we have $X_0 = n$. First observe that $(X_i \mid X_{i-1} = y) \sim B(y,1/2)$, so 
\[\E[X_i \mid X_{i-1} = y] = \E[B(y,1/2)] = \frac{1}{2} \cdot y \tag{1}\]
We use the fact that for any two random variables $X$ and $Y$, $\E[X] = \E_y[\E[X \mid Y = y]]$. This combined with $(1)$ gives
\[\E[X_i] = \E_y[\E[X_i \mid X_{i-1} = y]] = \E_y[1/2 \cdot y] =\frac{1}{2} \cdot \E[X_{i-1}] = \frac{1}{4} \cdot \E[X_{i-2}] = \cdots = \left(\frac{1}{2}\right)^i \cdot n\]
In particular, consider $D = c \cdot \log_{2}n$ for $c \geq 3$. We have that
\[\E[X_D] = \left(\frac{1}{2}\right)^{D} \cdot n = \frac{n}{n^c} = \frac{1}{n^{c-1}} \tag{2}\]
Now, by $(2)$ and Markov's inequality
\[\Pr[a \text{ participates in more than $D$ recursive calls}] = \Pr[X_D > 1] \leq \frac{\E[X_D]}{1} = \frac{1}{n^{c-1}}\]
Applying the union bound,
\begin{align*}
    \Pr[\text{PRp has depth greater than $c\cdot\log_{2}n$}] &= \Pr[\text{some } a \text{ participates in more than $D$ recursive calls}] \\
    &\leq \frac{n}{n^{c-1}} = \frac{1}{n^{c-2}}.
\end{align*}
as desired.
\end{proof}

==> Sections/msf.tex <==
\section{Minimum Spanning Forest Oracle}
\subsection{Introduction}
Let $G = (V,E,w_E)$ be a weighted undirected graph with weight function $w_E$. We denote $n = |V|$ and $m = |E|$. We assume that $G$ is given in compressed sparse row (CSR) format (see section \ref{csrref} for details). We make the additional assumption that the maximum edge weight in $G$ can be represented with $k\log n$ bits for some constant $k$. 

We note that the minimum spanning forest (MSF) for $G$ is unique under the assumption that ties are broken consistently. A \emph{minimum spanning forest oracle} supports queries that take as input an edge and return true if that edge is in the unique MSF for $G$. A \emph{connectivity oracle} supports queries that take as input a vertex and return the label of the connected component of $G$ that contains the vertex. The goal of this section is to describe a strong PIP algorithm to compute and encode an MSF oracle for $G$. More formally we will prove the following theorem.

\begin{thm} \label{graphthm}
    Given a graph with $n$ vertices and $m$ edges, an MSF oracle for the graph can be computed in $O(m\poly n)$ work and $O(\poly n)$ span whp. Moreover, whp we require only $O(\log^2 n)$ sequential stack space to compute such an oracle. Querying the oracle takes $O(\poly n)$ work and span whp.
\end{thm}

Additionally, we will show how to use an MSF oracle for $G$ to get a connectivity oracle for $G$. Thus, we also prove the below theorem.

\begin{thm} \label{conthm}
    Given a graph with $n$ vertices and $m$ edges, a connectivity oracle for the graph can be computed in $O(m\poly n)$ work and $O(\poly n)$ span whp. Moreover, whp we require only $O(\log^2 n)$ sequential stack space to compute such an oracle. Querying the oracle takes $O(\poly n)$ work and span whp.
\end{thm}

\subsection{Background and overview}
In \cite{2021pip}, the authors give a relaxed PIP algorithm to compute an MSF oracle for $G$ using $O(m^{1+\epsilon}\poly n)$ expected work, $O(m^{\epsilon}\poly n)$ span whp, and $O(m^{1-\epsilon})$ auxiliary space \cite{2021pip}. Additionally, querying the oracle takes $O(m^{\epsilon}\log n)$ expected time. They accomplish this by extending the notion of an implicit decomposition \cite{bendavid2017implicitdecompositionwriteefficientconnectivity} to the MSF problem. Motivated by this approach, we will define a new type of implicit decomposition which we refer to as an implicit prim decomposition. Then, using a block encoding scheme on the offset array of the CSR representation for $G$, we will be able to generate and encode a prim decomposition for $G$ with $O(n/\log n)$ centers. Then in a similar manner to \cite{2021pip}, we use Boruvka's algorithm to compute and encode an MSF across the centers of the implicit prim decomposition.

% We start with an overview of their approach. Their algorithm first generates an implicit decomposition of $G$ using an approach similar to \cite{bendavid2017implicitdecompositionwriteefficientconnectivity}. Next, the algorithm computes the MSF across these centers using a parallelization of Boruvka's algorithm. See section 6 of \cite{2021pip} for details. To query if an edge belongs to the MSF for $G$, the clusters of its endpoints are determined using a sequential prim-like search. Such a search requires $O(m^{\epsilon}\log n)$ time in expectation. If the endpoints belong to different clusters, i.e. the edge is a cut edge in the decomposition, the edge is simply checked for membership in the computed MSF across the centers. If instead the endpoints belong to the same cluster, the same prim-like search is used to determine if the edge belongs to the MST of the cluster and thus also belongs to the MSF for the whole graph. Note it is also possible that the edge belongs to a connected component without any centers, however it is easy to show that such components are small, $O(m^{\epsilon})$ in expectation, in which case it is possible to directly compute the MSF for the entire component.

% We now give an overview of our approach to the problem. An analysis of the algorithm above shows that by increasing the number of centers of the implicit decomposition, it is possible to achieve better work and span. Towards that end, we introduce a new type of implicit graph decomposition. This decomposition has similar theoretical guarantees to the implicit decomposition used in \cite{2021pip} and more importantly is amenable to encoding. Particularly, we will show how to encode an implicit graph decomposition with $O(n/{\log n})$ centers. Further, by modifying the Boruvka's algorithm mentioned above, we can construct and encode an MSF across the centers of the implicit graph decomposition. We will encode information by applying a block encoding scheme within the offset array (part of the CSR representation) for $G$.



\subsection{Facilitating encoding}\label{csrref}
As mentioned in the introduction to this section, we assume that $G$ is given in CSR format. That is, $G$ is represented by an array, say $I$, of $n + 4m + 1$ elements where $I[0]$ stores the number of vertices in $G$, the next $n$ elements store $n$ offsets (one per vertex) to the location in $I$ of the last neighbor for each vertex, and finally the last $4m$ elements are reserved for storing neighbor list and weights. Let $A = I[1:n]$ represent the offset list of $I$, and $B = I[n+1:n + 4m]$ represent the edge list. Note that the offset array provides a unique labeling of vertices from $1$ to $n$. We will use this labeling to break ties in a consistent manner. Specifically, we can generate a lexicographical ordering of the edges in $G$ using a pairing function on the unique vertex labels of each endpoint.

% If $(u,v)$ is an edge of $G$ with weight $x$ and $v$ is the $k$th pair in $u$'s edge list, we read this from $I$ as $B[(A[u] - A[u-1])/2 + k] = (v,x)$. Note that $A[u]-A[u-1]$ is the number of elements in the slice of $B$ that contains $u$'s neighbors. We divide by 2 since each consecutive pair contains information for a single edge. Let $i = (A[u] - A[u-1])/2 + k$.

Observe that $A$ is sorted. We will make the additional assumption that $G$ contains no degree $0$ vertices so that all the numbers in $A$ are distinct.
% We note it is possible to remove this assumption through a preprocessing step (see [?]).
We can therefore block $A$ into $\lfloor n/b\rfloor$ blocks each of size $b$, for some block size $b = O(\log n)$, and apply inversion encoding within the blocks. We note the last block may actually be larger than $b$. Since our algorithm will be correct under the assumption that each block can use $\lfloor b/2 \rfloor$ pairs of elements for encoding, we can simply ignore the extra pairs contained in the last block. As discussed in section \ref{encodingdisc}, this scheme allows us to encode a fixed amount of numbers and a fixed amount of bits in each block. Also, due to the initial sorted state of $A$, we can always accurately read the $i$th element of the offset array by checking if it is inverted with the other element in its pair.

\subsubsection{Notation} Let $p$ be a vertex. We denote the neighbor list of $p$ in $B$ as $N_p$ where $|N_p| = A[p] - A[p-1]$ and iteration over $N_p$ is done edge wise i.e. $r \in N_p[0] = (v,x)$ where $v$ is adjacent to $p$ with weight $x$.

% , i.e. the position in $E$ of the last neighbor for the $i$th vertex.

\subsection{Graph decomposition}\label{graphdecomp}

The blocking structure we described above naturally gives a way to decompose the graph. In each block of $A$, we independently and uniformly at random choose a vertex and encode its label using consecutive pairs in the block. Let $S$ denote the set of chosen vertices and $S_B$ the corresponding encoding in $A$. Then observe that $S$ induces a decomposition of $G$ given by the collection $\{C_s \colon s \in S\}$  where $C_s$ consists of the vertices of $V$ that are closest to $s$ when traversing the graph in a Prim-like fashion. More formally, define $T(v,k)$ as the sub-tree of $G$ generated after running Prim's algorithm \cite{10.5555/1614191} rooted at $v$ for $k$ iterations, i.e. after visiting $k$ vertices. Then $v \in C_s$ if and only if $s = \min_{k} T(v,k) \cap S \not= \emptyset$. We say that $C_s$ is a \emph{cluster} in the decomposition with \emph{center} $s$. We refer to the set of centers together with their induced clusters as the \emph{Prim decomposition} of $G$. As in \cite{bendavid2017implicitdecompositionwriteefficientconnectivity}, we define the \emph{cluster graph} as the multigraph $G'$ whose vertex set is the set of centers $S$ and edge set consist of all the edges in $E$ that cut across two distinct clusters.

Next, we prove an important correctness lemma: 


\textcolor{red}{break}
 
% More formally, $G' = (S, \langle \{u,v\} \in E \colon u \in C_s \text{ and } v \in C_{s'}, \text{ where } s \not= s' \rangle)$. 
In the remainder of this section, we discuss how to facilitate the computation of the MSF on the implicit cluster graph $G'$. 


\subsection{Center Search}
Since we do not explicitly store the cluster graph, we need a method to determine which edges are in $G'$. We use a prim-like search to determine the closest centers and thus the clusters of its endpoints, and check that they are distinct. This search is sequential and uses a standard implementation of the priority queue and set data structures. These data structures can be stored in the local stack of the thread executing the search. In order to guarantee $O(\log ^2 n)$ sequential stack-allocated usage, we require that the queue and set never contain more than $c' \log^2 n$ vertices for some constant $c'$. Towards that end, we process a vertex $v$ by adding it to the set and adding the $c'\log^2 n$ vertices in $v$'s neighborhood with smallest edge weight to the queue. If the queue size goes over $c'\log^2 n$ vertices, only the $c'\log^2 n$ distinct vertices of smallest weight are kept. To guarantee the search is correct, we keep track of the smallest edge weight evicted from the queue. We only ever add vertices with edge weight smaller than this value. Once the set reaches its maximum allowed size or the queue becomes empty, if a center has not been found, we start over with the new requirement that the max size of the queue and set is $2c'\log^2 n$. We iterate this procedure until a center is found. Later, we show that whp we never iterate the search more than once. Before giving the pseudocode for the search, we note that as a preprocessing step we sort the edge list of each vertex. If the edge list is $O(\log n)$ we can use a simple in-place sequential sorting algorithm like bubble sort. Otherwise, we can do this with the parallel in-place merge sort algorithm from section \ref{ipmerge}. The work and span for this step are bounded above by $O(n \log n)$ and $O(\log^3 n \log \log n)$ respectively.
% This will allow us to add the closest $O(\log^2 n)$ vertices to the queue without having to do repetitive sorts of edge lists.
Note that this preprocessing step has no effect on the encoding scheme since we only use $A$ to do encoding.
The pseudocode for the search is given below. \\

\begin{algorithm2e}[H]
% \SetKwFor{For}{for}{}{do}{}
\caption{Center Search}{\label{Center Search}}
    \DontPrintSemicolon
    \textbf{Input: } A graph $G = (V,E,w_E)$ in CSR format, a set of centers $S_B$, iteration number $k$, and a starting vertex $u$ \\
    \textbf{Output: } The closest center to $u$\\
    $\mathcal{Q} \gets \{(u,0)\}$ \Comment{$\mathcal{Q}$ is a priority queue}\\
    $\mathcal{V} \gets \{u\}$ \Comment{$\mathcal{V}$ represents the visited set} \\
    $t \gets \infty$ \Comment{$t$ stores the smallest edge weight evicted from $\mathcal{Q}$} \\
    $L \gets 2^kc' \log^2 n$ \Comment{max queue and set size} \\
    \While{$\mathcal{Q} \not= \emptyset$ \text{ and } $|\mathcal{V}| \leq L$} {
        $(p,x) \gets \text{pop}(\mathcal{Q})$ \Comment{$p$ is a vertex and $x$ is a weight} \\
        \text{insert}$(\mathcal{V},p)$ \\
        \lIf(\Comment{$p$ is a center}){$p = S_B[\lfloor p/b \rfloor]$} {\textbf{return} $p$}
        \For{$r \in N_p[0:\min(|N_p|,L)]$} {
            \lIf{$w_E(p,r) < t$}{
                insert$(\mathcal{Q},(r, w_E(p,r)))$ 
            }
        }
        \lIf{$|\mathcal{Q}| > L$}{retain only $L$ vertices with smallest edge weight and update $t$ if necessary}
    }
    % repeat if center not found with $k+1$.
\end{algorithm2e}

% \begin{algorithm2e}[t]
% % \SetKwFor{For}{for}{}{do}{}
% \caption{Center Search}{\label{Center Search}}
%     \DontPrintSemicolon
%     \textbf{Input: } A graph $I = (n,A,B)$ in CSR format, a set of centers $S$, iteration number $k$, and a starting vertex $u$ \\
%     \textbf{Output: } The closest center to $u$\\
%     $\mathcal{Q} \gets \{(u,0)\}$ \Comment{$\mathcal{Q}$ is a priority queue}\\
%     $t \gets \infty$ \Comment{$t$ stores the smallest path weight evicted from $\mathcal{Q}$} \\
%     $L \gets 2^kc' \log^2 n$ \Comment{max queue size} \\
%     \While{$\mathcal{Q} \not= \emptyset$} {
%         $(p,x) \gets \text{pop}(\mathcal{Q})$ \Comment{$p$ is a vertex and $x$ is a weight} \\
%         \lIf{$p \in S$} {\textbf{return} $p$}
%         \For{$i \gets 0$ to $\min((A[p]-A[p-1])/2,2L)$} {
%             $k \gets \min((A[p]-A[p-1])/2,2L) - i$ \\
%             \If{$x + B[k][1] < t$}{
%             insert$(\mathcal{Q},(B[k][0],B[k][1] + x))$ \Comment{recall $B[k] = (r,x')$ for some $r,x'$}
%             }
%         }
%         \lIf{$|\mathcal{Q}| > L$}{retain only $L$ closest vertices to $u$ and update $t$ if necessary}
%     }
%     % repeat if center not found with $k+1$.
% \end{algorithm2e}




For iteration $(k+1)$, Center Search takes a starting vertex and an iteration variable set to $k$ and returns the closest center within $2^kc' \log^2 n$ vertices if it exists. If not, then the search is started again with the iteration variable incremented by $1$. Note that if Center Search does not find a center and $t = \infty$ and $|\mathcal{V}|$, then we can identify $u$ as belonging to a connected component of $G$ with no centers. We note that in line 10, $\lfloor p/b \rfloor$ is the index of the block containing the vertex with label $p$. We will use this notation throughout the rest of the section.

Next we analyze the time complexity of the first iteration of Center Search and show that whp we find the closest center from the starting vertex in this iteration. In each round of the search we process a vertex $p$, add $p$ to the visited set, and insert at most $c'\log^2 n$ of $p$'s neighbors into a priority queue. Given that the queue has size at most $c'\log^2 n$, each insertion takes time $O(\log^2 n \log\log n)$. The queue eviction (line 13) similarly requires only $O(\log^2 n \log\log n)$ time. Adding a vertex to the visited set (line 9) requires $O(\log\log n)$ time. Finally, to determine if $p$ is a center, we use the ReadBlock function given in section \ref{encodingdisc}, which takes $O(\log\log n)$ span and $O(\log n)$ work. In total, a round of Center Search requires $O(\log^2 n \log\log n)$ time. To bound the total time of Center Search, it will be sufficient to give an appropriate tail bound for the number of vertices traversed. Fix a starting vertex $v$ and let $S_{v,L}$ be the random variable which represents the number of vertices traversed by a Center Search starting at $v$ with max queue and set size $L$. We show in the section \ref{primanalysis} of the appendix that $\Pr[S_{v,L} \geq b \cdot (c\log n + 1)] \leq \frac{1}{n^c}$. As $b \leq  r \log n$ for some constant $r$, the tail bound gives that whp, the closest center to $v$ is within the $r(c+1)\log^2 n$ closest vertices to $v$. Therefore, the total time for the first iteration of Center Search is $O(\log^4 n \log\log n)$. Further, by taking $c' = r(c+1)$ we see that whp we need only iterate Center Search once. Note that this analysis shows that the size of a connected component of $G$ that contains no center is $O(\log^2 n)$ whp. 

% To close the section, we note that under the bounded degree assumption, that is every vertex has degree at most some constant $d$, the time complexity of Center Search can be greatly reduced. Indeed, since every vertex has degree at most $d$, by taking $L = dr(c+1)\log^2 n$ whp we only iterate the search once and furthermore, the time complexity of the search is simply $O(\log^2 \log\log n)$.

To close the section, we note that once we have fixed a set of centers, the runtime of center search is determined by the starting vertex. Thus, by a simple union bound, we deduce with high probability that every Center Search terminates in $O(\log^4 n \log \log n)$ time.
% We will then use this MSF across the decomposition to produce an MSF oracle for the graph $G$, in an analogous way to that described in subsection 5.2. 

\subsection{MSF for the cluster graph}\label{msfclutergraph} In the previous section, we showed how to use Center Search to identify $G'$. We can now use Boruvka's algorithm to compute an MSF for $G'$. 

To implement Boruvka's algorithm for $G'$, we use a union-find data structure \cite{UnionFind} where each node stores the label of a vertex in $G'$, a parent pointer, two flag bits, and an edge (the source, target, and weight) in the MSF for $G'$. We denote these $L_B$,$P_B$,$C_B$, and $E_B$. For notational convenience, we denote the source, target, and weight stored by $E_B[i]$ as $E_B[i][0]$,$E_B[i][1]$, and $E_B[i][2]$ respectively.  We adopt the standard sequential find operation and use a randomized star contraction to perform parallel forest contractions. Note that the inverted trees in this structure represent the connected components in Boruvka's algorithm and the roots of these trees represent the corresponding representatives. $C_B$ is used to determine if a node is the root of an inverted tree and $D_B$ is used during the forest contraction. We denote the described data structure as $R_B$.

Recall that in each block of $A$, we need to encode the label of a center in the implicit prim decomposition. Since the centers correspond exactly to the vertices in $G'$, and thus the labels of nodes $R$ we have $L_B = S_B$. It is natural to encode the remaining associated data for each node in the same block. Note that by assumption edge weights in $G$ can be represented by $\log n$ bits. Rather than use inversion encoding to store the MSF edge information of each node in $R_B$, we will overwrite the first three elements of each block and encode the values stored there at the end of the block. We do this to avoid the use atomic operations on slices since in each Boruvka's round, we need to concurrently read and write to $E_B$. Since we are not actually encoding $E_B$ we drop the $B$ subscript going forward. Take $b = 10\log n + 7$. We now specify the encoding used by each block of $A$. The first $3$ elements of block $i$ will be used to store $E[i]$. Then the next $4\log n$ pairs of block $i$ in $A$ are used to encode $S_B[i],P_B[i]$, the next 4 pairs are used to used to encode $C_B[i]$ and $D_B[i]$ respectively, and finally the last $6\log n$ pairs are needed to encode the original offsets stored in the first three elements of block $i$.

We start with every cluster being in its own component. To represent this we set the first three elements of every block to $-1$ and initialize the remaining parts of $R_B$ with the WriteBlock function to set the source and destination to $-1$ and flip the root bit to true. We then iterate Boruvka's rounds until the inverted trees of $R_B$ represents the connected components of $G'$. In each Boruvka's round we need to identify $G'$. We do this by iterating in parallel over the edges of $G$, and using the Center Search algorithm to determine which edges are edges in $G'$. Note that to iterate over $E$, we will iterate over the offset array and then for each vertex iterate over its neighbor list. For threads that are assigned to the one of the first three elements of a block in $A$, the offset value will need to be read using the ReadBlock function on the corresponding pairs at the end of the block. Below we give pseudocode for a Boruvka round.

\begin{algorithm2e}[H]
\SetKwFor{ParFor}{parallel for}{do}{endfch}
\SetKwBlock{DoParallel}{do in parallel}{end}
\DontPrintSemicolon
\caption{find}
\textbf{Input: } A graph $G = (V,E,w_E)$ in CSR format, a union-find data structure $R_B$, and a center $s$ \\
\textbf{Output: } the root of the inverted tree in $R_B$ containing $s$ \\

$t \gets s$ \\
\While(\Comment{$t$ is not the root}){$!C_B[\lfloor t/b \rfloor]$}{
    $t \gets P_B[\lfloor t/b \rfloor]$ \Comment{traverse to the parent of $t$}
}
\textbf{return} $t$
\end{algorithm2e}

\begin{algorithm2e}[H]
\SetKwFor{ParFor}{parallel for}{do}{endfch}
\SetKwBlock{DoParallel}{do in parallel}{end}
\DontPrintSemicolon
%\SetKwFor{For}{for}{}{do}{}
\caption{Boruvka Round}{\label{clusterBoruvka}}
    \textbf{Input: } A graph $G = (V,E,w_E)$ in CSR format, a union-find data structure $R_B$, and a bit in shared memory $t$ \\
    $t \gets 1$ \Comment{$t$ is a flag} \\
    \ParFor(\Comment{vertex with label $i$}){$i \gets 1$ to $n$}{
        % $k \gets (A[i] - A[i-1])/2$ \\
        \ParFor{$e = (j,w_E(\{i,j\})) \in N_i$}{
            $s_1 \gets $ Center Search from vertex $i$ $\parallel$ \\
            $s_2 \gets$ Center Search from $j$ \\ 
            \If(\Comment{edge in $G'$}){$s_1 \not= s_2$} { 
                $r_1 \gets $ find($R_B,s_1$) $\parallel$ \\
                $r_2 \gets $ find($R_B,s_2$)\\
                \If{$r_1 \not= r_2$}{
                    Use a compare-and-swap operation to atomically update $E[\lfloor r_1/b \rfloor]$ and $E[\lfloor r_2/b \rfloor]$ \\ to be the minimum between the current stored edge weight and $w_E(i,j)$. If either \\ root node is updated, set $t$ to $0$.
                }
            }
        }
    }
\end{algorithm2e}

After a Boruvka round, the root nodes of $R_B$ together with the edges of $G'$ stored in these nodes form a forest. Particularly, they represent the forest computed by Boruvka's algorithm at the corresponding stage on $G'$. We note that the bit $t$ is set to $0$ if the edge stored by a root node is updated (line 11-13). $t$ will be used to determine when Boruvka's algorithm is finished. We perform forest contraction in parallel through randomized star contraction. The pseudocode for a round of this procedure is given below.

\begin{algorithm2e}[H]
\SetKwFor{ParFor}{parallel for}{do}{endfch}
\SetKwFor{ParForEach}{parallel for each}{do}{endfch}
%\SetKwFor{For}{for}{}{do}{}
\caption{Forest Contraction Round}{\label{fContract}}
    \DontPrintSemicolon
    \textbf{Input: } A graph $G = (V,E,w_E)$ in CSR format and a union-find data structure $R_B$ \\
    \ParForEach(\Comment{$i$ ranges over $0,\dots,n/b-1$}){$S_B[i]$}{
        \If(\Comment{$S_B[i]$ is a root of an inverted tree in $R_B$}){$C_B[i] = 1$}{
            $D_B[i] \overset{R}{\gets} \{0,1\}$
        }
    }

    \ParForEach{$S_B[i]$}{
        \If{$C_B[i] = 1$}{
            $s' \gets E[i][1]$ \Comment{adjacency of vertex $S_B[i]$} \\
            $r' \gets$ find$(R_B,s')$ \Comment{root of $s'$ in $R_B$} \\
            \If(\Comment{$S_B[i]$ has an adjacency in $F'$ }){$r'$ is not $-1$}{
                \If{$D_B[i] = 0$ and $D_B[\lfloor r'/n \rfloor] = 1$}{
                    $P_B[i] \gets r'$ \\
                    $C_B[i] \gets 0$ \\
                }
            }
        }
    }
\end{algorithm2e}

 Algorithm \ref{fContract} performs a round of forest contraction on by linking together inverted trees of $R_B$. In more detail, if the edge stored by $r_1$ points to $r_2$ then we want to link the inverted tree with root $r_1$ to the inverted tree with root $r_2$, i.e. set $r_2$ as the parent of $r_1$. However, if $r_2$ also points to $r_1$ then there is conflict. We break the symmetry in a similar manner to that of section \ref{tphasemerge}. That is, in each round, each root node of $R_B$ Then $r_1$ contracts to $r_2$ if $r_1$ flipped tails ($D_B[r_1] = 0$) and $r_2$ flipped heads ($D_B[r_2] = 1$) (lines 10-12).  

 We can now combine Algorithm \ref{clusterBoruvka} and Algorithm \ref{fContract} to perform a parallel Boruvka's algorithm on $G'$ and encode a data structure for answering MSF queries on $G$ within the offset array $A$. As mentioned above we iterate Boruvka's rounds until the inverted trees of $R_B$ contain an MSF for $G'$. That is each round, starts by performing Algorithm \ref{clusterBoruvka} and then iterating Algorithm \ref{fContract} until no root node in $R_B$ stores an edge of $G'$ that points to another root node, i.e. the inverted trees of $R_B$ represent the isolated connected components. We can determine when to stop the iteration using a bit $t'$ in shared memory in a similar fashion to the Done function given in section \ref{merge-transformation-phase}. Similarly we can use a bit $t$ to determine when Boruvka's algorithm has finished.

We now analyze the complexity of this Algorithm. Our algorithm has the same structure of the sequential Boruvka's algorithm in that each iteration reduces the number of inverted trees (connected components) by at least half. Therefore, we need only iterate at most $O(\log n)$ times. As a consequence to this, the height on any inverted tree in $R_B$ is also upper bounded by $O(\log n)$ and so every find operation takes time $O(\log n)$. Then the work and span of each Boruvka Round is dominated by the $m$ Center Searches each taking $O(\log^4 n \log\log n)$ time whp (see the discussion at the end of section \ref{graphdecomp}). There is an additional cost of $\log n + \log m$ span to fork $n + m$ threads assuming binary forking. Thus overall each Boruvka round takes $O(m\log^4 \log\log n)$ work and $O(\log^4 \log\log n)$ span whp. Next, each Forest Contraction Round requires $\log n$ span and $O(n)$ work to fork $n$ threads and each thread does a constant time operation. So the time complexity of the forest contraction is determined by the number of iterations of the inner while loop (line 7). A standard probabilistic analysis using a union bound shows that whp the number of iterations is bounded by $\log n$. Thus the overall complexity of the forest contraction is $O(\log^2 n)$ span and $O(n\log n)$ work whp. Putting everything together, our Algorithm computes an MSF for $G'$ in $O(m\log^5 n\log\log n) = O(m\poly n)$ work and $O(\log^5 \log\log n) = O(\poly n)$ span whp.


% We recall Boruvka's algorithm. Given an undirected weighted graph $G = (V,E,w_E)$, let $F$ be the forest with vertex set $V$ and no edges. We refer to this forest as the \emph{Boruvka forest}. Every connected component of $F$ has a vertex that acts as the representative for the component. In what follows, it is understood that operations on connected components of $F$ are done through representatives. The algorithm begins by finding the minimum-weight edge incident to each vertex in $G$ and adding these edges to $F$. Then, it repeats a similar process by finding for each connected component in $F$, the minimum-weight outgoing edge of the corresponding component in $G$, and adding these edges to $F$. After each Boruvka round, every connected component in $F$ is either adjacent to another connected component or it is isolated. To remove these adjacencies, the algorithm performs a forest contraction on $F$. Each repetition of this process reduces the number of nonisolated connected components in $F$ to at most half the former value, so after logarithmically many repetitions the process finishes. At termination, $F$ will represent a unique (assuming consistent tie breaking) MSF for $G$.

% To implement Boruvka's algorithm for $G'$, we represent the Boruvka forest $F'$ with a union-find data structure \cite{UnionFind} where each node stores the label of a vertex in $G'$, a parent pointer, two flag bits, and an edge of the MSF for $G'$. We denote these $L_B$,$P_B$,$C_B$, and $E_B$. We adopt the standard sequential find operation and later give a parallel forest contraction algorithm. The inverted trees in this structure represent the connected components of the forest $F'$ and the roots of these trees represent the corresponding representatives. $C_B$ is used to determine if a node is the root of an inverted tree and $D_B$ is used during the forest contraction. We denote the described data structure as $R_B$. Then it is clear that $R_B$ contains a representation of $F'$. In the remainder of this section, we discuss how $R_B$ is encoded in $A$ and give a parallel Boruvka's algorithm to compute the MSF for $G'$ using $R_B$.
% \textcolor{red}{something about the way "representatives for connectd components" are being talked about is confusing}





% First we give the pseudocode for a parallel Boruvka round and some useful auxiliary functions.



% \begin{algorithm2e}[H]
% \SetKwFor{ParFor}{parallel for}{do}{endfch}
% \SetKwBlock{DoParallel}{do in parallel}{end}
% \DontPrintSemicolon
% \caption{update}
% \textbf{Input: } A graph $G = (V,E,w_E)$ in CSR format, a union-find data structure $R_B$, a root $r$, an edge $e = (i,j,w_E\{i,j\})$, and a bit in shared memory $t$ \\
% \textbf{Output: } updated edge information stored by $r$

% $w \gets E_B[\lfloor r/b \rfloor][2]$ \Comment{weight of edge stored by $r$} \\
% $u \gets E_B[\lfloor r/b \rfloor][1]$ \Comment{target of edge stored by $r$} \\
% $v \gets E_B[\lfloor r/b \rfloor][0]$ \Comment{source of edge stored by $r$} \\


% \If{$w > w_E(i,j)$}{
%     $E_B[\lfloor r/b \rfloor][2] \gets w_E(i,j)$ \\
%     $E_B[\lfloor r/b \rfloor][1] \gets j$ \\
%     $E_B[\lfloor r/b \rfloor][0] \gets i$ \\
%     $t \gets 0$
% }

% \If{$w = w_E(i,j)$}{
%     $k = \frac{1}{2}(u + v)(u + v + 1) + v$ \Comment{Cantor pairing function} \\
%     $k' = \frac{1}{2}(i + j)(i + j + 1) + j$ \\
%     \If(\Comment{$e$ is lexicographically smaller than the edge stored by $r$}){$k > k'$}{
%     $E_B[\lfloor r/b \rfloor][2] \gets w_E(i,j)$ \\
%     $E_B[\lfloor r/b \rfloor][1] \gets j$ \\
%     $E_B[\lfloor r/b \rfloor][0] \gets i$ \\
%     $t \gets 0$
%     }
% }

% \end{algorithm2e}





% \begin{algorithm2e}[h]
% \SetKwFor{ParFor}{parallel for}{do}{endfch}
% \SetKwBlock{DoParallel}{do in parallel}{end}
% \DontPrintSemicolon
% %\SetKwFor{For}{for}{}{do}{}
% \caption{Boruvka Round}{\label{clusterBoruvka}}
%     \textbf{Input: } A graph $I = (n,A,B)$ in CSR format and a union-find data structure $R$ \\
%     \ParFor{$i \gets 0$ to $n-1$}{
%         $k \gets (A[i] - A[i-1])/2$ \\
%         \ParFor{$j \gets 0$ to $k$}{
%             $s_1 \gets $ Center Search starting at vertex $i$ $\parallel$ \\
%             $s_2 \gets$ Center Search starting at vertex $B[k+j][0]$ \\ 
%             \If(\Comment{edge in $G'$}){$s_1 \not= s_2$} { 
%                 $r_1 \gets $ find($R,s_1$) $\parallel$ \\
%                 $r_2 \gets $ find($R,s_2$)\\
%                 \If(\Comment{edge in $F'$}){$r_1 \not= r_2$}{
%                     In parallel, update the edges stored by $r_1$ and $r_2$ to store the \\ minimum between the current edges and $(i,j)$.
%                 }
%             }
%         }
%     }
% \end{algorithm2e}

% In a Boruvka Round we find the minimum outgoing edge from each connected component in $F'$, i.e. the minimum outgoing edge of each inverted tree in $R_B$. We start by iterating in parallel over the edges of $G$, and using the Center Search algorithm to determine which edges are edges in $G'$ (lines 2-7). Then for those edges in $G'$, we use $R_B$ to determine if they belong to $F'$, i.e. the edge is incident to two distinct connected components (lines 8-10). The final lines of Algorithm \ref{clusterBoruvka} deserve a more complete discussion. Fix an edge $(i,j,w_E(i,j))$ and adopt the same notations given in the algorithm. In line 11, we read the weight of the current edge stored by node $r_1$ and compare it to $w_E(i,j)$. If the weight is $-1$, i.e. the node is not storing an edge currently, or smaller we attempt to write the edge $(i,j,w_E(i,j))$ to node $r_1$. The same process is done for node $r_2$ (line 12). Since these lines are happening in parallel for all the edges incident to the connected component represented by $r_1$, the read and write operations are concurrent and potentially overlap each other. The situation is further complicated by the presence of encoding. We discuss how to handle the concurrency for Algorithm \ref{clusterBoruvka} in section \ref{concurrencytalk}. We note that the bit $t$ is set to $0$ if the edge stored by a root node is updated (line 10,18 in update). $t$ will be used to determine when Boruvka's algorithm is finished.

% After a Boruvka round, the root nodes of $R_B$ together with the edges of $G'$ stored in these nodes form a forest. Particularly, they represent $F'$ at the corresponding stage of Boruvka's algorithm on $G'$. We perform forest contraction in parallel through randomized star contraction. The pseudocode for a round of this procedure is given below.


    
    
    % \While{
    %     some root stores an edge to another root
    % }{
    %     \ParFor{roots $r \in R$}{
    %         Set random bit stored by $r$ to random number from $\{0,1\}$
    %     }
    %     \ParFor{roots $r \in R$}{
    %         $r' \gets $ other vertex of edge stored by $r$ \\
    %         \If{random bit stored by $r'$ is 1 and random bit stored by $r$ is 0} {add edge from $r$ to $r'$, and set root bit of $r$ to 0}
    %     }
    % }
    % \ParFor{}{}


% Algorithm \ref{fContract} performs a round of forest contraction on $F'$ by linking together inverted trees of $R_B$. In more detail, if the edge stored by $r_1$ points to $r_2$ then we want to link the inverted tree with root $r_1$ to the inverted tree with root $r_2$, i.e. set $r_2$ as the parent of $r_1$. However, if $r_2$ also points to $r_1$ then there is conflict. We break the symmetry in a similar manner to that of section \ref{tphasemerge}. That is, in each round, each root node of $R_B$ Then $r_1$ contracts to $r_2$ if $r_1$ flipped tails ($D_B[r_1] = 0$) and $r_2$ flipped heads ($D_B[r_2] = 1$) (lines 10-12).  


% Below is the pseudocode for computing an MSF for $G'$.

% {
% \setlength{\interspacetitleruled}{0pt}%
% \setlength{\algotitleheightrule}{0pt} 
% \begin{algorithm2e}[H]
% \DontPrintSemicolon
% \SetKwFor{ParForEach}{parallel for each}{do}{endfch}
% \Fn{$\mathrm{Contracted}$} {
% \textbf{Input:} A graph $G = (V,E,w_E)$ in CSR format, a union-find data structure $R_B$, and a bit in shared memory \\
% \ParForEach{$S_B[i]$}{
%     \If(\Comment{$S_B[i]$ is a root node}){$C_B[i] = 1$}{
%         \If(\Comment{$S_B[i]$ points to another root node}){$C_B[\lfloor E_B[i][1] \rfloor] = 1$ and $t = 1$}{
%             $t \gets 0$
%         }
%     }
% }
% }
% \end{algorithm2e}
% }
% \begin{algorithm2e}[H]
% \SetKwFor{ParFor}{parallel for}{do}{endfch}
% \SetKwBlock{DoParallel}{do in parallel}{end}
% \DontPrintSemicolon
% \caption{MSF for $G'$}\label{msfclusteralg}
% \textbf{Input: } A graph $G = (V,E,w_E)$ in CSR format and an initialized union-find data structure $R_B$. \\
% \textbf{Output: } The MSF of $G'$ encoded in the offset array $A$ \\ 

% $t_1 \gets 1$ \Comment{bit stored in the heap} \\
% $t_2 \gets 1$ \Comment{bit stored in the heap} \\

% \While{$t_1 = 1$}{
%     Perform a Boruvka Round on $G$ and $R_B$ using bit $t_1$ to detect termination \\
%     \While{$t_2 = 1$}{
%         Perform a Forest Contraction Round on $G$ and $R_B$ using bit $t_2$ to detect termination
%     }
%     $t_2 \gets 1$ \Comment{reset flag} 
% }
% \end{algorithm2e}

% Algorithm \ref{msfclusteralg} combines Algorithm \ref{clusterBoruvka} and Algorithm \ref{fContract} to perform a parallel Boruvka's algorithm on $G'$ and encode a data structure for answering MSF queries on $G$ within the offset array $A$. Each round of the outer while loop (line 5) starts by performing a Boruvka round and then iterating forest contraction rounds until no root node in $R_B$ stores an edge of $G'$ that points to another root node, i.e. the inverted trees of $R_B$ represent the isolated connected components of $F'$ after performing a forest contraction (lines 7-8). We can determine when to stop the iteration using a bit $t_2$ (line 4) in shared memory in a similar fashion to the Done function given in section \ref{merge-transformation-phase}. Similarly we can use a bit $t_1$ to determine when Boruvka's algorithm has finished (line 4).

% We now analyze the complexity of Algorithm \ref{msfclusteralg}. Our algorithm has the same structure of the sequential Boruvka's algorithm in that each iteration of the outer while loop reduces the number of inverted trees (connected components) by at least half. Therefore, we iterate the outer while loop at most $O(\log n)$ times. As a consequence to this, the height on any inverted tree in $R_B$ is also upper bounded by $O(\log n)$ and so every find operation takes time $O(\log n)$. Then the work and span of each Boruvka Round is dominated by the $m$ Center Searches each taking $O(\log^4 n \log\log n)$ time whp (see the discussion at the end of section \ref{graphdecomp}). There is an additional cost of $\log n + \log m$ span to fork $n + m$ threads assuming binary forking. Thus overall each Boruvka round takes $O(m\log^4 \log\log n)$ work and $O(\log^4 \log\log n)$ span whp. Next, each Forest Contraction Round requires $\log n$ span and $O(n)$ work to fork $n$ threads and each thread does a constant time operation. So the time complexity of the forest contraction is determined by the number of iterations of the inner while loop (line 7). A standard probabilistic analysis using a union bound shows that whp the number of iterations is bounded by $\log n$. Thus the overall complexity of the forest contraction is $O(\log^2 n)$ span and $O(n\log n)$ work whp. Putting everything together, Algorithm \ref{msfclusteralg} computes an MSF for $G'$ in $O(m\log^5 n\log\log n) = O(m\poly n)$ work and $O(\log^5 \log\log n) = O(\poly n)$ span whp.


% We now analyze the complexity. Each vertex experiences a logarithmic number of contractions whp so the maximum height of a tree in the final union find structure is logarithmic. Thus with high probability every find operation always takes at most $\log n$ time. Each Boruvka round does $m$ Center Searches and $m$ find operations. There is complexity associated to updating the minimum edge weight, and the corresponding implications on the complexity are discussed in the following section. Each forest contraction round has logarithmic depth and $O(n/\log n)$ work.




% \noindent\textcolor{red}{nonsense below}









% gives $((k+3)\log n + 2)$ pairs in which we can apply inversion encoding to encode the required number of bits.



\subsection{Strong PIP MSF oracle} Combining the results of the last two sections gives us an MSF oracle for $G$. Indeed, generate an implicit graph decomposition and compute and encode $R_B$ within the offset array $A$. Now given a query $e = (v,u) \in E$, we execute Center Search from each endpoint. If the endpoints of $e$ belong to different clusters and $e$ is part of the MSF for $G'$, then some node in $R_B$ witnesses this. Specifically, if $C_u$ contains $u$ and $C_v$ contains $v$ then $s_u$ and $s_v$ (the centers of $C_u$ and $C_v$) are leaves in $R_B$ and $e$ must be stored in some node along the path from $s_u$ or $s_v$ to the roots of their respective inverted trees in $R_B$. Since the height of the inverted trees in $R_B$ is bounded by $\log n$ and reading $E$ and $P_B$ at each node is a $\log \log n$ span and work operation, the total time to check if $e$ is in the MSF for $G'$, and hence the MSF for $G$, is $O(\log n \log \log n)$. Now, if $s_u = s_v$, i.e. $u$ and $v$ belong to the same cluster, we can check if $e$ is encountered during the Center Search from $u$. Since Center Search traverses the same edges as a Prim Search starting from $u$, it will traverse along MSF edges of $G$ until it finds a center. Thus $e$ is in the MSF for $G$ if and only if it appears in the traversal of Center Search starting at $u$. From the analysis in section \ref{graphdecomp}, the Center Search will find $s_u$ in $O(\log^4\log\log n)$ time whp. Finally, it is also possible that $e$ belongs to a connected component of $G$ with no centers. As noted in the end section \ref{graphdecomp}, such components have size $O(\log ^2 n)$ whp. Therefore, we can simply iterate Center Search from $u$ until we exhaust the component ($t = \infty$ and $|\mathcal{V}| > L$). Overall, we see that the oracle requires at most $O(\poly n)$ time. Additionally, by the analysis in section \ref{msfclutergraph}, computing $R_B$ requires $O(m\poly n)$ work and $O(\poly n)$ span whp and $O(\log^2 n)$ sequential stack-allocated space. Thus we conclude Theorem \ref{graphthm}.


% \subsection{Handling concurrency}\label{concurrencytalk} In this section we discuss how to handle the concurrency present in Algorithm \ref{clusterBoruvka}. Excluding these lines, the only meaningful concurrency (potential overlap in concurrent read and write operations) present in our algorithm is the bit used to determine when Boruvka's algorithm should terminate. There however, we don't require the use of primitive atomic operations like compare-and-swap (CAS) since the order in which writes take effect has no effect on the correctness of the computation. Now recall our discussion after Algorithm \ref{clusterBoruvka}. Each Boruvka round starts by forking $n$ thread. Each thread then conducts a number of reads on $I$ through executing Center searches (lines 4-5). The threads processing edges belonging to $G'$ next perform find operations (lines 8-9). Finally, the threads processing edges connecting two root nodes of $R_B$ perform the update function (lines 10-11). Since these threads are operating in parallel over the shared memory of $I$, there is a potential for overlapping concurrent read and write operations. To better understand the scenario, fix the $i$th of $A$. Per our discussions in sections \ref{csrref} and \ref{msfclutergraph}, this block encodes the label of a vertex $s$ in $G'$ (a center), the label of a parent node $p$ for $s$ in the inverted tree containing $s$, the source $u$, target $v$, and weight $w_E(u,v)$ of an edge in $G'$, and finally two bits. Observe that the only slice of the block in which reads and writes can overlap consist of the pairs that encode the edge stored by node $s$. Then to remove the potential overlap, we alter the encoding scheme. We take the block size to be $b = 2(k+4)\log n + k + 6$. Then the first $k+2$ elements of each block will act as a buffer of $(k+2)\log n$ bits to store the edge information for node $s$, the next $4\log n$ pairs will encode $s$ and $p$, the next $2(k+2)\log n$ pairs will encode the original $k$ values of the block, and finally the last $4$ pairs encode the two bits. We remark that we need at most $k+2$ elements of each block to act as a buffer due to the somewhat weak assumption on the maximum edge weight. Now to perform reads and writes on the edge information stored by a node, we can use a CAS operation on the on the buffer in the corresponding block. We can also modify the Boruvka Round algorithm and Forest Contraction Round algorithm to work with the new encoding scheme by directing any read on one of the first $k+2$ elements of a block to the corresponding slice whose pairs encode the original value. Since $k$ is a constant, the algorithms runtime remains the same.

\subsection{Strong PIP connectivity oracle} We note that its easy to extend our algorithm to compute an MSF oracle for $G$ to compute a connectivity oracle of $G$. Recall that a connectivity oracle supports queries that take as input a vertex and return the label of the connected component of $G$ that contains the vertex. To compute a connectivity oracle for $G$, we generate an implicit prim decomposition and compute $R_B$. Then given a vertex $v$, we run Center Search starting form $v$ and keep track of the minimum label of a vertex encountered during the search. If a center is found, say $s_u$, then $s_u$ is a leaf in $R_B$. We traverse along the path from $s_u$ to the root of the inverted tree in $R_B$ that contains $s_u$ and return the label of the root. Otherwise $u$ is part of a connected component with no centers and the minimum label seen serves as the connected component label for $u$. The connectivity oracle construction has the same work and span as the MSF oracle construction. Thus we conclude Theorem \ref{conthm}.



% \subsection{Boruvka Record}

% The main ideas of Boruvka's algorithm in computing the MSF across a decomposition are as follows: Initially we have a graph $M$ with vertex set all the clusters and no edges. In rounds, we find the minimum outgoing edges from the components of each vertex of the graph, then add the edges to the $M$, and contract the endpoints of those edges. We repeat the rounds until there are no edges between components of vertices in the graph. We are ultimately left with the MSF across the decomposition. We do the contraction using star contraction. To determine which clusters an edge is between, we perform a prim-like search from each endpoint of the edge to find the corresponding centers (and thus the corresponding cluster).

% We see that to each cluster $C_s$ we need to associate the following data:
% \begin{enumerate}
%     \item the center of the cluster, $s$
%     \item the current minimum outgoing edge, minEdge$[s]$
%     \item whether or not the cluster is contracted, isContracted$[s]$
%     \item which cluster this cluster is contracted to, contractedTo$[s]$
%     \item a bit for use in star contraction, coin$[s]$
% \end{enumerate}
% As mentioned in the previous subsection, the centers for our decomposition naturally correspond to blocks. Hence we can encode all the above data corresponding to a cluster in the block corresponding to its center.

% Our variant of Boruvka's algorithm is then as follows. First, initialize all minimum outgoing edges to null to -1 and all contracted states to false.

% For each uncontracted cluster, find the minimum outgoing edge of the corresponding component and store it in minEdge$[s]$. Do this by iterating in parallel over the edge list. For each edge $e$, do prim-searches out from both endpoints and find the closest centers $s_1$ and $s_2$. Then find the corresponding components $C_{s_1'}$ and $C_{s_2'}$ of $s_1$ and $s_2$ by traversing along contractedTo$[s_i]$ until the corresponding cluster is not contracted. Then set minEdge$[s_i']$ to be min$($minEdge$[s_i'], e)$.

% Now repeat the following procedure until the uncontracted clusters form a forest with the current edges: In parallel, for each uncontracted cluster $C_s$, flip a random coin and store the result in coin$[s]$. Again in parallel, for each uncontracted cluster $C_s$, if $C_{s'}$ is not contracted, where $s'$ is the component of the other endpoint of minEdge$[s]$, and coin$[s] = 0$ and coin$[s'] = 1$, set contractedTo$[s']$ equal to $C_s$ and set isContracted$[s]$ to true.

% Repeat the last two paragraphs until no component has edges to any other component. At the end of this process, the graph formed by minEdge$[s]$ is the MSF across the decomposition.

% We call the data stored in all the blocks a \emph{Boruvka record}, since it is essentially a record of what happens throughout this verision of Boruvka's algorithm.





% \newpage
% \subsection{nonsense}


% \begin{defn}
%     An \emph{MSF oracle} for a graph $G$ answers queries of the form ``is $e \in F_G$?''
% \end{defn}



% Ultimately, the work and span of this algorithm are determined by the number of centers in the implicit decomposition. To see this, observe that the algorithm in \cite{2021pip} enumerates $O(\log n)$ Boruvka rounds (whp) and in each round a prim-like search is done from each endpoint of each edge in the graph. The purpose of this search is to find, for each endpoint of an edge, the cluster of the implicit decomposition that contains it. The complexity of the search is given by the number of vertices traversed multiplied by an $O(\log n)$ insertion cost from the use of a priority queue. The number of vertices traversed by the search follows a geometric distribution with parameter $1/m^\epsilon$. Thus, in expectation, the time complexity of one search is $O(m^\epsilon\log n)$ and so the total expected work done by all the searches in a Boruvka round is $O(m^{1+\epsilon}\log n)$. Since the searches are done in parallel, the span of a Boruvka round is simply $O(m^\epsilon\log n)$ in expectation. 




% From the above analysis, it is clear that the work and span of the algorithm are dominated by the time complexity of the prim-like search, which in turn is determined by the number of vertices traversed \textcolor{red}{in a prim search}. Further, as seen above, this number follows a geometric distribution whose parameter is equal to the probability of a vertex being a center. In \cite{2021pip} this is given by $1/m^\epsilon$. Suppose we take the sampling probability to instead be $1 / \log n$. Then the expected number of vertices traversed would simply be $\log n$. Plugging this into the above analysis we get $O(m \log^2 n)$ expected work and $O(\log^2 n)$ expected span for a Boruvka round. Despite the vastly improved work and span bounds of this approach, there is an obvious problem. That of course being the fact that the algorithm given by this approach no longer satisfies the conditions of the relaxed PIP model. Indeed, using $1/\log n$ as the probability of sampling a center, we get the expected number of centers as $n/\log n$, which is larger than $n^\epsilon$ for every $\epsilon < 1$. We resolve this problem by choosing to encode auxiliary data for the centers and MSF edges across these centers within the input. To facilitate this encoding we need to specify an input format for $G$ and modify the algorithm given by \cite{2021pip}. The actual encoding will be done in a manner similar to section 4, where we block the input and apply inversion encoding within the blocks. Before describing the details of our algorithm, we note that this approach not only improves the work and span bounds of our algorithm but also ensures that it satisfies the requirements of the strong PIP model. 

% We assume that $G$ is given in compressed sparse row format (CSR). That is, $G$ is represented by an array, say $A$, of $n + 4m + 1$ elements where $A[1]$ stores the number of vertices in $G$, the next $n$ elements store $n$ offsets (one per vertex) to the location in $A$ of the last neighbor for each vertex, and finally the last $4m$ elements are reserved for storing neighbor list and weights. Let $V = A[2:n+1]$ represent the offset list of $A$, and $E = A[n+1:n + 4m + 1]$ represent the edge list. We can equivalently view $E$ as an array of $2m$ pairs where each pair represents a vertex and edge weight. We will adopt this view going forward. Note that $V$ provides a unique labeling of vertices from $1$ to $n$. We will use this labeling to break ties in a consistent manner. Finally, we assume that the maximum edge weight present in $G$ is less than $n^k$ where $k$ is an even positive integer.

% We block $V$ (the offset array) into $n/b$ blocks of size $b$. Each block will encode the vertex label of a center in the implicit decomposition and an edge of the MSF for the decomposition.





% For completeness, we define the implicit decomposition below.

% \begin{defn}\label{implicitdecomp}
%     Given a subset $S$ of $V$, the \emph{implicit decomposition} of $G$ induced by $S$ is the collection $\{C_s : s \in S\}$ where $C_s$ consists of the vertices of $V$ closest to $s$. We say that each $C_s$ is a \emph{cluster} in the implicit decomposition with \emph{center} $s$.
% \end{defn}



% \begin{defn}
%     Let $S$ be as in Definition \ref{implicitdecomp}. Define the \emph{contraction} $G_S$ as the graph whose vertex set is given by the set of centers $S$. The edges of $G_S$ consist of all edges in $G$ that cross between clusters. More formally, $G_S = (S, E_S)$ where $E_S = \{(u,v) \in E : u \in C_{s_i} \text{ and } v \in C_{s_j}, \text{ where } i \not= j\}$.
% \end{defn}

% We call $G_S$ the contraction because it is the graph obtained by contracting each cluster in $G$ and ignoring the connected components of $G$ which do not contain any center.

% \begin{clm}{\label{msf-oracle-decomp}}
%     Given an MSF oracle for the contraction $G_S$, we can compute an MSF oracle for $G$.
% \end{clm}
% \begin{proof}
%     Let $e = (u,v)$ be an edge of $G$. Additionally, let $G'$ denote the connected component of $G$ that contains $e$ and $G_S'$ the restriction of the contraction of $G$ to $G'$. From each endpoint, we can determine its closest center in $G'$ using a prim-like search. If no such centers exist, we compute the MST of $G'$, say $T_{G'}$, and check if $e \in T_{G'}$. Otherwise, there is at least one center in $G'$. Observe that in any connected component of $G$ with at least one center, the clusters in the implicit decomposition of that component will form a partition. It follows then, that the MST for $G'$ is given by the union of the MST for $G'$, and the MSTs for the clusters of $S$ in $G'$. Now if $u$ and $v$ belong to distinct clusters we can query the MSF oracle for $G_S$ to determine if $e \in T_{G_S}$ and hence in the MST for $G'$. If not, then $u$ and $v$ belong to the same cluster, say $C_i$. Observe that when searching out to $i$ from $u$ and $v$, the use of the Prim-like search enforces that only edges of the minimum spanning tree for $C_i$ are used in the traversal. Thus, $e \in T_{G'}$ if and only if $e \in T_{C_i}$ if and only if its contained in the search paths from $u$ and $v$ to $i$.
% \end{proof}

% Claim \ref{msf-oracle-decomp} reduces the computation of an MSF oracle for $G$ to choosing an appropriate $S$ and computing an MSF oracle for $G_S$.



% This section will show how to compute and encode an MSF oracle of a graph using only $O(\log^2 n)$ sequential stack-allocated space whp. We accomplish this by improving the relaxed PIP algorithm by Gu et al. \cite{2021pip} that computes such a data structure using $O(m^{1+\epsilon}\log^2 n)$ expected work and $O(m^{\epsilon}\poly n)$ span whp.






% \begin{thm}
%     Given a graph with $n$ vertices and $m$ edges, an MSF oracle for the graph can be computed in $O(m\poly n)$ expected work and $O(\poly n)$ span whp. Moreover, whp we require only $O(\log^2 n)$ sequential stack space to compute such an oracle. Querying the oracle takes $O(\poly n)$ work and span whp.
% \end{thm}


% \newpage

% \subsection{Towards constructing an MSF oracle}

% We start with the following definition.



% Naturally, a representation of $T_G$ as a data structure is an MSF oracle for $G$. However, such a data structure is likely to have a high space complexity (in most cases $\Omega(n)$). We seek a way of computing a space efficient and encodable MSF oracle for $G$. Towards that end, we use the notion of an implicit decomposition \cite{bendavid2017implicitdecompositionwriteefficientconnectivity}.


% The efficiency of the reduction depends on the implicit decomposition and 
% method of search used to find the centers. We start with the details of the search algorithm. As in our proof, we use a prim-like search when finding a vertex's closest center. The details of the search algorithm are given below.

% \begin{algorithm2e}[h]
% \caption{Center Search}{\label{Center Search}}
%     \DontPrintSemicolon
%     \textbf{Input: } A graph $G = (V,E,w_E)$, a set of centers $S$, and a starting vertex $u$ \\
%     \textbf{Output: } The closest center to $u$\\
%     $\mathcal{Q} \gets \{(0,u)\}$ \Comment{$\mathcal{Q}$ is a priority queue}\\
%     \While{$\mathcal{Q} \not= \emptyset$} {
%         $(x,p) \gets \text{pop}(\mathcal{Q})$\\
%         \lIf{$p \in S$} {\textbf{return} $p$}
%         \For{$r \in N(p)$} {
%             insert($\mathcal{Q}$, $r$, $x + w_E(p,r)$) 
%         }
%     }
% \end{algorithm2e}
% \newpage

% The Center Search algorithm is prim-like in the sense that it will visit vertices in the same order as Prim's algorithm until the closest center is found. As given, we cannot get any meaningful bounds on the space complexity of Algorithm \ref{Center Search}. Indeed, in the worst case, the priority queue could contain $n-1$ vertices. Furthermore, the time complexity of Center Search depends entirely on the implicit decomposition. In section [?] we will discuss how to modify Algorithm \ref{Center Search} and choose an appropriate implicit decomposition.


% Up to this point, our approach is essentially identical to that in [?], though presented slightly differently. The reason for our difference in presentation is that we emphasize that having the contraction oracle is sufficient to solve the problem. We will see that we can construct an oracle for the contraction using $O(|S|)$ space. We will give a method for choosing $S$ so that the size $|S| = C n/\log n$ is deterministic. Since the oracle is small enough, we will be able to encode it directly in the input and thus make the algorithm in place.

% \subsection{Constructing the oracle}
% Fix a graph $H$. We describe a data structure, which we call a \emph{Boruvka record}, that gives an MSF oracle for $H$. The Boruvka record $B_H$ is a DAG with vertex set $V(H)$. Additionally, each vertex stores the weight and endpoints of an MSF edge $E_u$, and a flag representing the contraction state of the vertex. \\ \\ \\ \\


% The Boruvka record is defined through performing Boruvkas algorithm. The initial state of the Boruvka record is given by the forest with vertex set $V(H)$. Further, every vertex stores an empty MSF edge and its contraction state is set to false. Upon running the first Boruvka round, the minimum outgoing edge from vertex $u$ is computed and stored in the corresponding records of its node. Next, in the contraction stage, if $u$ is contracted to the vertex $v$, we set the contraction state of $u$ to true, and add the directed edge $(u,v)$ to the DAG. \\ \\ \\ \\ 


% We continue iterating this construction, where the difference is that $E_u$ will store the minimum outgoing edge of the contracted part corresponding to the vertex $u$. Also, when adding the edge during the contracted step, note that the edge added is between the two vertices corresponding to the contracted parts which the endpoints the MSF edge are part of. \textcolor{blue}{Last two sentences need to be rewritten and expanded upon}


% \noindent\fbox{\parbox{\dimexpr \linewidth-2\fboxsep-2\fboxrule}{

% Boruvka's algorithm:

% (1) Boruvka round: For each uncontracted vertex find minimum outgoing edge of the corresponding component and store it in $E_u$. If $E_u = \{u,v\}$, find the uncontracted vertex $v'$ whose component contains $v$ (this can be done by iterating out in the DAG from $v$ til a vertex has no out-edges).

% (2) Contraction step: Repeat the following procedure until we get a forest of points on the current MSF edges: For each uncontracted vertex $u$, flip a bit and store the result in a bit $b_u$ corresponding to that vertex. For each uncontracted vertex $u$, if $v'$ is not contracted and $b_u = 0$ and $b_{v'} = 1$, add an edge in the DAG from $u$ to $v'$, and set the vertex $u$ to be contracted.

% Repeat (1) followed by (2) until all uncontracted vertices form a forest.

% }}

% Given a Boruvka record, we get an oracle for MSF. Given an edge $e = \{u,v\} \in E(H)$, we can determine if $e \in T_H$ as follows:  For both $u$ and $v$, do the following. Check if $E_u = e$. If so, return yes. Otherwise, traverse the DAG to the next vertex and repeat. Repeat until we get to a uncontracted vertex (i.e. the vertex corresponding to the contraction of the entire connected component of $u$), in which case return false. If this procedure for both $u$ and $v$ returns false, return no. The runtime for this query depends only on the depth of the DAG which will be logarithmic with star contraction. (\textcolor{red}{Prove this})

% Fix a set of centers $S$.
% First observe that we can easily adapt Boruvka's algorithm to compute the Boruvka record of the contraction graph $G_S$ just by using $G$ directly.
% Note the size of $B_{G_S}$ is $O(|S|)$ since each vertex has a constant amount of data associated to it and the depth will be $O(\log |S|)$.

% \subsection{Facilitating encoding}

%  % We assume that $G$ is given in compressed sparse row format (CSR). That is, $G$ is represented by an array, say $A$, of $n + 4m + 1$ elements where $A[1]$ stores the number of vertices in $G$, the next $n$ elements store $n$ offsets (one per vertex) to the location in $A$ of the last neighbor for each vertex, and finally the last $4m$ elements are reserved for storing neighbor list and weights. Let $V = A[2:n+1]$ represent the offset list of $A$, and $E = A[n+1:n + 4m + 1]$ represent the edge list. \textcolor{blue}{abuse of notation?} We can equivalently view $E$ as an array of $2m$ pairs where each pair represents a vertex and edge weight. We will adopt this view going foward. Note that $V$ provides a unique labeling of vertices from $1$ to $n$. We will use this labeling to break ties in a consistent manner. Finally, we assume that the maximum edge weight present in $G$ is less than $n^k$ where $k$ is an even positive integer.

% \textcolor{red}{Describe how to interpret Boruvka record as an array (this should be easy)} This sets up the Boruvka record part of the algorithm. The only remaining part to describe is how we choose $S$.

% Earlier, we remarked that the set of centers heavily influences the runtime of our algorithm. Not only this, but to facilitate the encoding we need to choose $S$ wisely so that we can encode the Boruvka record in a computable way always. We cannot simply do the naive method of having each vertex be in $S$ randomly with probablity $p$ for a fixed choice of $p$, since in such a case, the size of $S$ is not deterministic so there is not a clear ``universal'' way of encoding the Boruvka record. This is what is done in [?] so cannot be adapted to our setting; we need to something smarter to get an in-place algorithm. 

% A key observation is that if the set of centers has a fixed size then there is a natural way of encoding the structure.

% We want to choose a set of centers $S$ with $|S|$ deterministically depending on $n$, while still having $S$ be distributed well enough so that the runtime of the algorithm stays low. We want as many centers as possible to minimize work, while still being amenable to encoding; it turns out that $n/\log n$ is the natural choice, as we shall see. The key insight to how we choose the centers is that if we partition the vertex set into sets of size $\log n$ and form $S$ by choosing a single center randomly from each partition, then everything works out well; this does not even depend on the particular partition (see the appendix, \textcolor{red}{though should probably state the consequence for runtime here}). This is good because there are natural ``computable'' partitions of the vertex set of a graph in CSR format by taking consecutive slices of the offset array of size $C  \log n$ where $C$ is a constant. Part of the reason this is natural, is because we can encode the data of a center $c$ and its associated data in the Boruvka record in the slice corresponding to $c$.

% \subsection{Doing the encoding}

% \textcolor{red}{Write how the natural partition gives a natural way to do the encoding.}

% \subsection{Slight modifications to Boruvka to support encoding}

% \textcolor{red}{Describe how to do tricky part of Boruvka round (write min).}

% \textcolor{red}{Done????}
% \textcolor{blue}{No.}


% \subsection{Notation and Assumptions}
% We assume that $G$ is given in compressed sparse row format (CSR). That is, $G$ is represented by an array, say $A$, of $n + 4m + 1$ elements where $A[0]$ stores the number of vertices in $G$, the next $n$ elements store $n$ offsets (one per vertex) to the location in $A$ of the last neighbor for each vertex, and finally the last $4m$ elements are reserved for storing neighbor list and weights. Define $O = A[1:n]$ to represent the offset list of $A$, and $N = A[n:n + 4m + 1]$ to represent the edge list. We can equivalently view $N$ as an array of $2m$ pairs where each pair represents a vertex and edge weight. Note that $O$ provides a unique labeling of vertices from $1$ to $n$. Finally, we assume that the maximum edge weight present in $G$ is less than $n^k$ where $k$ is an even positive integer.

% \subsection{???} Let $b$ be a positive integer, where $b < n$. For simplicity, we assume $b$ divides $n$ evenly, though this assumption is easily removed. Then partition $O$ into $n/b$ blocks and denote them as $B^1,B^2,\dots, B^{n/b}$. Within each block, select uniformly at random a vertex as a center. Denote the vertex chosen in block $B^j$ as $c_j$. Together, the set $C = \{c_j : 1 \leq j \leq n/b\}$ induces an implicit decomposition of $G$. We equip each cluster with a constant amount of auxiliary space that will be used to store a cluster's center id, an edge of the MSF, and a flag that is set true if the cluster is contracted. Note that it is possible that there will be connected components of $G$ that do not contain centers. However, by consequence of the construction, such connected components are small and easy to process.

% Our algorithm will continue in a manner similar to the relaxed PIP MSF algorithm given by Gu et al [citation]. We will proceed by computing an MSF over the clusters of the implicit decomposition using a parallel variant of Borůvka's algorithm. We start with each cluster being in its own component. A round of our algorithm will consist of two stages.
% \newpage
